Distributed Optimization with Consensus Constraint for Multi-Robot Semantic Octree Mapping

This work develops a distributed optimization algorithm for multi-robot 3-D semantic mapping using streaming range and visual observations and single-hop communication. Our approach relies on gradient-based optimization of the observation log-likelihood of each robot subject to a map consensus constraint to build a common multi-class map of the environment. This formulation leads to closed-form updates which resemble Bayes rule with one-hop prior averaging. To reduce the amount of information exchanged among the robots, we utilize an octree data structure that compresses the multi-class map distribution using adaptive-resolution.

==> tex/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we presented a distributed multi-class mapping algorithm that enables online construction of a semantic octree map of an unknown environment using a team of mobile robots. The globally consistent map can be accessed via a query from any of the robots, eliminating the need for a central estimation unit. Such a common map can be utilized by robots for exploration and planning. In a future work, we couple our proposed multi-robot mapping algorithm with a distributed planning method over the space of $\text{SE}(3)$ robot poses in order to achieve multi-robot exploration.
